DualGAN: Unsupervised Dual Learning for Image-to-Image Translation

Conditional Generative Adversarial Networks (GANs) for cross-domain image-to-image translation have made much progress recently. Depending on the task complexity, thousands to millions of labeled image pairs are needed to train a conditional GAN. However, human labeling is expensive, even impractical, and large quantities of data may not always be available. Inspired by dual learning from natural language translation, we develop a novel dual-GAN mechanism, which enables image translators to be trained from two sets of unlabeled images from two domains. In our architecture, the primal GAN learns to translate images from domain U to those in domain V, while the dual GAN learns to invert the task. The closed loop made by the primal and dual tasks allows images from either domain to be translated and then reconstructed. Hence a loss function that accounts for the reconstruction error of images can be used to train the translators. Experiments on multiple image translation tasks with unlabeled data show considerable performance gain of DualGAN over a single GAN. For some tasks, DualGAN can even achieve comparable or slightly better results than conditional GAN trained on fully labeled data.

==> introduction_zl.tex <==
\section{Introduction}
\label{sec:intro}

Many image processing and computer vision tasks, e.g., edge detection, image segmentation, 
stylization, and abstraction, can be posed as image-to-image translation problems~\cite{isola2016image}, 
which convert one visual representation of an object or scene into another. Conventionally, these tasks have 
been tackled separately due to their intrinsic 
disparities~\cite{ledig2016photo,li2016precomputed,wang2016generative,mathieu2015deep,isola2016image,taigman2016unsupervised}. 


It is not until the past two years that general-purpose and end-to-end deep learning frameworks, most notably those utilizing fully convolutional networks (FCNs)~\cite{long2015fully} and conditional generative adversarial nets (cGANs)~\cite{isola2016image}, have been developed to enable a {\em unified\/} treatment of these tasks.


Up to date, these general-purpose methods have all been supervised and trained with a large number of
 {\em labeled\/} and {\em matching\/} image {\em pairs\/}. In practice however, acquiring
such training data can be time-consuming (e.g., with pixelwise or patchwise labeling) and even unrealistic. 
For example, while there are plenty of photos or sketches available, photo-sketch image pairs depicting the same persons under the same poses are scarce. In some other situations, such as \zl{aerial image to map conversion. can we change it to day-night conversion?}, even though labeled and matching image pairs can be obtained, they are not accurately aligned and may contain slightly different contents.

% For example, for day scene$\rightarrow$night scene conversion, image pairs could be easily acquired using stationary cameras. However, image pairs that contain exactly the same contents (e.g., moving objects, fog, clouds, and lights) are rare.} 
%These two situations also apply to many other tasks such as \zl{artistic stylization of images, and transferring material across objects.}


In this paper, we aim to develop an {\em unsupervised\/} learning framework for general-purpose
image-to-image translation, which only relies on {\em unlabeled\/} image data, such as two sets of 
photos and sketches for the photo-to-sketch conversion task. The obvious technical challenge is
how to train a translator without any data characterizing correct translations. Our approach is inspired
by {\em dual learning\/} from natural language processing~\cite{xia2016dual}. Dual learning trains 
{\em two\/} ``opposite'' language translators (e.g., English-to-French and French-to-English) 
simultaneously by minimizing the {\em reconstruction loss\/} resulting from a {\em nested\/} application 
of the two translators. The two translators represent a primal-dual pair and the nested 
application forms a closed loop, allowing \zl{a sophisticated reconstruction loss to be applied}. Specifically, the
reconstruction loss measured over monolingual data (either English or French) would generate informative 
feedback to train a bilingual translation model.


%Addressing all the problems mentioned above, we propose a novel unsupervised dual learning architecture 
%which targets on general-purpose image-to-image translation. 

%The original dual learning work~\cite{xia2016dual} enables training of bilingual translations with 
%unlabeled monolingual data only. In the dual learning paradigm~\cite{xia2016dual}, the primal task 
%(English-to-French translation) and the dual task (French-to-English translation) form a closed loop, 
%so that the English (French) monolingual data can be translated to French (English), and then reconstructed to English (French). 

Our work develops a dual learning framework for image-to-image translation for the first time and differs
from the original NLP dual learning method of Xia et al.~\cite{xia2016dual} in two main aspects. First, 
the NLP method relied on pre-trained (English and French) language models to indicate how confident 
the outputs of translators are natural sentences in its own language. With 
general-purpose processing in mind and the realization that such pre-trained models are difficult to 
obtain for many image translation tasks, our work develops GAN discriminators~\cite{goodfellow2014generative} 
that are trained adversarially with the translators to capture domain distributions. Hence, we call our
learning architecture {\em DualGAN\/}. Furthermore, we employ FCNs as translators which naturally accommodate the 2D structure of images, rather than sequence-to-sequence translation models such as LSTM or GUT.


Taking two sets of unlabeled images as input, each representing an image domain, DualGAN simultaneously 
learns two reliable image translators from one domain to the other and hence can operate on a wide variety of image-to-image translation tasks. Its effectiveness is validated through comparison with both the original GAN and conditional GAN~\cite{isola2016image}. The comparison results demonstrate that for some applications, DualGAN can outperform supervised methods trained on labeled data.

